Understanding the Complexity of Lifted Inference and Asymmetric Weighted Model Counting

In this paper we study lifted inference for the Weighted First-Order Model Counting problem (WFOMC), which counts the assignments that satisfy a given sentence in first-order logic (FOL); it has applications in Statistical Relational Learning (SRL) and Probabilistic Databases (PDB). We present several results. First, we describe a lifted inference algorithm that generalizes prior approaches in SRL and PDB. Second, we provide a novel dichotomy result for a non-trivial fragment of FO CNF sentences, showing that for each sentence the WFOMC problem is either in PTIME or #P-hard in the size of the input domain; we prove that, in the first case our algorithm solves the WFOMC problem in PTIME, and in the second case it fails. Third, we present several properties of the algorithm. Finally, we discuss limitations of lifted inference for symmetric probabilistic databases (where the weights of ground literals depend only on the relation name, and not on the constants of the domain), and prove the impossibility of a dichotomy result for the complexity of probabilistic inference for the entire language FOL.

==> complexity.tex <==
% !TEX root =  paper.tex

%%%%%%%%%%%%%%%%%%%%%%%
%%%% \input{exampleProof}
%%%%%%%%%%%%%%%%%%%%%%%



==> proofOfTheorem1.tex <==
% !TEX root =  complexity.tex
\subsection{Proof of Theorem \ref{thm:type1}}

\label{subsec:proofOfTheorem_1}

\subsubsection{Outline}

We start by considering a concrete example to demonstrate the hardness proof.
\[
Q = (R(x) \lor \lnot S(x,y) \lor T(y))(\lnot R(x) \lor S(x,y) \lor \lnot T(y))
\]

We prove that the \#P-hard 
problem, Positive Partitioned 2-CNF \citep{provan1983complexity}, can be solved
in polynomial time by consulting an oracle for $P(Q)$.

The steps are:

\begin{itemize}

	\item Encode $\Phi$ into a structure with the unary predicates
			$R$ and $T$ and the binary predicate $S$
			
	\item Assign probabilities to the tuples such that, by
			consulting an oracle for $P(Q)$ a polynomial number of times,
			we construct a system of equations from which we can extract
			the number of satisfying assignments of $\Phi$ in polynomial
			time
	
\end{itemize}

We first define $\Phi$, an instance of PP2CNF. Given two disjoint sets of
Boolean variables $X_1, \dots, X_{n_1}$ and $Y_1, \dots, Y_{n_2}$ and a
bipartite graph $E \subseteq [n_1] \times [n_2]$, the positive, partitioned
2-CNF formula defined by $E$ is:
\[
\Phi = \bigwedge_{(i, j) \in E} (X_i \lor Y_j)
\]
$\#\Phi$ is the problem of counting the number of satisfying assignments of 
$\Phi$. \citep{provan1983complexity} show that this problem is
\#P-hard. 

In the following we assume, without loss of generality, that $n_1 = n_2$.

\subsubsection{Encoding $\#\Phi$}

Given $\Phi$, we construct a structure with unary predicates $R$ and $T$ and binary predicate $S$.
We set the active domain of the structure to be $[n]$.

We set the probabilities of the tuples as follows:

\[
P(R(i)) = x
\]

\[
P(T(j)) = y
\]

\[
P(S(i, j)) = \left\{
  \begin{array}{lr}
    a & \text{ if }(i, j) \in E \\
    b & \text{ if }(i, j) \not \in E
  \end{array}
\right.
\]


\subsubsection{Recovering $\#\Phi$}


Given a valuation $\theta$ of the variables in $\Phi$, denote $E_\theta$ the following event:
\begin{gather*}
E_\theta = \forall i.(R(i) = true \texttt{ iff } \theta(X_i) = true) \\
\land \forall j.(T(j) = true \texttt{ iff } \theta(Y_j) = true)
\end{gather*}

Note that $E_\theta$ completely fixes the unary predicates $R$ and $T$ and leaves $S$ unspecified.
The intuition behind this is that, given $E_\theta$, each Boolean variable corresponding to
$S(x,y)$ is now independent of every other $S(x', y')$. 
In general, given an assignment of $R(i)$ and $T(j)$, we examine the following four functions
that define the probability that the query is true on the branch $(i, j)$: \Eric{need to formalize this}
\begin{align*}
& F_1 = Q[R(i) = 0, T(j) = 0] \\
& F_2 = Q[R(i) = 0, T(j) = 1] \\
& F_3 = Q[R(i) = 1, T(j) = 0] \\
& F_4 = Q[R(i) = 1, T(j) = 1] \\
\end{align*}

For our example query $Q$, the functions are as follows:
\begin{align*}
& F_1 = \lnot S(i, j) \\
& F_2 = \text{true} \\
& F_3 = \text{true} \\
& F_4 = S(i,j) \\
\end{align*}

Denote $f_1, f_2, f_3, f_4$ the arithmetization of the corresponding Boolean formulas:
\begin{align*}
& f_1 = \left\{
  \begin{array}{lr}
    1-a & \text{ if }(i, j) \in E \\
    1-b & \text{ if }(i, j) \not \in E
  \end{array}
\right. \\
& f_2 = 1 \\
& f_3 = 1 \\
& f_4 =  \left\{
  \begin{array}{lr}
    a & \text{ if }(i, j) \in E \\
    b & \text{ if }(i, j) \not \in E
  \end{array}
\right. \
\end{align*}

For this example, we will ignore $f2$ and $f3$. 

Define the parameters of theta as:
\begin{align*}
& k = \text{number of $i$'s s.t. } R(i)=1 \\
& l = \text{number of $j$'s s.t. } T(j)=1 \\
& p = \text{number of $(i,j) \in E$ s.t. } R(i)=T(j)=1 \\
& q = \text{number of $(i,j) \in E$ s.t. } R(i)=T(j)=0
\end{align*}

\Eric{general form will have additional $r,s$ terms for
R = 1, T = 0 and vice versa}

We can now describe the probability of $Q$ given $E_\theta$.
\[
P(Q | E_\theta) = a^p (1-a)^q  b^{kl - p} (1-b)^{(n-k)(n-l) - q}
\]

We also have the following expression for $P(E_\theta)$:
\[
P(E_\theta) = x^k (1-x)^{n-k} y^l (1-y)^{n-l}
\]

Let $N(k,l,p,q) = $ number of $\theta$'s that have parameters $k,l,p,q$.
Combined with the above, we have:
\[
P(Q) =  (1-b)^{n^2} (1-x)^n (1-y)^n \sum_{k,l,p,q} T
\]

where:
\begin{align*}
T =  & N(k,l,p,q) \ast (a/b)^p [(1-a)/(1-b)]^q \\
&                    [x/(1-b)^n (1-x)]^k [y/(1-b)^n \\
&                    (1-y)]^l [b(1-b)]^{kl} \\
= &     N(k,l,p,q) \ast A^p B^q X^k Y^l C^{kl}
\end{align*}

Here $A,B,X,Y$ are independent, but $C$ is dependent on $A,B$. 
\Eric{ Can we omit the following equations?
\begin{align*}
& A = a/b \Rightarrow a = A \ast b \\
& B = (1-a)/(1-b) \Rightarrow 1-a = B*(1-b) \\
& \Rightarrow  1 = A*b + B - B*b \\
& \Rightarrow  b = (1-B)/(A-B) \\
& \Rightarrow  C = b*(1-b) = - (1-A)(1-B)/(A-B) \\
&      C =  - [(1-A)(1-B)] / (A-B)
\end{align*}
}

Next, we use an oracle for computing $P(Q)$ multiple times on structures 
with different probabilities $x, y, a, b$. The resulting matrix is invertible
by the lemmas of Section \ref{subsec:invertible}. Then we
solve for $N(k,l,p,q)$, for all values $k,l,p,q$.  From here, we
have $\#\Phi = \sum_{k,l,p} N(k,l,p,0)$ (that is, we count only those assignments
where $q = 0$, corresponding to assignments where every $(i, j) \in E$ is satisfied
by $X_i$ or $Y_j$). This completes the proof of hardness for query $Q$.

In order to generalize this proof, we 

\Eric{need to describe how $f_1,f_2,f_3,f_4$, along with $g_1,g_2,g_3,g_4$, go into $T$ -
probably easiest to redo the above formulas with these functions included from outset}


\Eric{Now we can construct a matrix of some size, whose determinant is non-zero by the 
lemmas of the following section. This allows us to solve for $p$ and $q$ in polynomial
time, and from this, recover the solution to $\#\Phi$.}


\subsubsection{Proving the Matrix is Invertible}
\label{subsec:invertible}

Let $M(m_1, m_2, n_1, n_2)$ be the matrix whose entries are:
\[
     A_u^p  \ast  B_v^q  \ast  X_w^k  \ast  Y_z \ast l  \ast  C_{uv}^{kl}
\]

    where the row is $(p,q,k,l)$ and column is $(u,v,w,z)$
    and the ranges are:
\begin{align*}
&         p,u = 0,..,m_1-1 \\
&         q,v = 0,..,m_2-1 \\
&         k,w = 0,..,n_1-1 \\
&         l,z = 0,..,n_2-1 \\
\end{align*}

We denote the Vandermonde determinant:  $V(X) = \prod_{k,k'}(X_k - X_{k'})$

\begin{lemma}If $m_1=m_2=1$ then
\[
   det(M) = C_{00}^{n_1 \ast n_2 \ast (n_1-1) \ast (n_2-1)/4}  \ast  V^{n_2}(X)  \ast n_1 V^{n_1}(Y)
\]
\end{lemma}
\begin{proof} 
The matrix $M(1,1,n_1,n_2)$ has the following entries:
\[
        X_w^k  \ast  Y_z \ast l  \ast  C_{00}^{kl}
\]
   
All elements in row $(k,l)$ have the common factor $C_{00}^{kl}$.  After
we factorize it from each row, the remaining matrix is a Kroenecker
product of two Vandermonde matrices.
\end{proof}


\begin{lemma}
\begin{gather*}
   det(M(m_1, m_2, n_1, n_2)) = \\
       \prod_{u > 0}(A_u - A_0)^{m_2 \ast n_1 \ast n_2} \\
        \ast  det(M(1, m_2, n_1, n_2)) \\
        \ast  det(M(m_1-1, m_2, n_1, n_2))
\end{gather*}

Where in $M(m_1-1, m_2, n_1, n_2)$ instead of $A_0, \dots, A_{m_1-2}$ we have
$A_1, \dots, A_{m_1-1}$, i.e. the index $u$ is shifted by one, and similarly
in $C_{uv}$ the index $u$ is shifted by one.
\end{lemma}

\begin{proof}
We eliminate $A_0$, similarly to how we would eliminate it from
a Vandermonde matrix: subtract from row $(p+1,q,k,l)$ the row $(p,q,k,l)$
multiplied by $A_0$; do this bottom up, and cancel $A_0$ in all rows,
except the rows of the form $(0,q,k,l)$.  We only need to be careful
that, when we cancel $A_0$ in row $(p+1, q, k, l)$ we use the same $q,k,l$
to determine the row $(p,q,k,l)$.

For an illustration we show below these two rows $(p,q,k,l)$ and
$(p+1,q,k,l)$, and the two columns, $(0, v0, w0, z0)$ and $(u,v,w,z)$:

In the original matrix:
\[
\begin{pmatrix}
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\dots & T_1 & \dots & T_2 & \dots \\
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\dots & T_3 & \dots & T_4 & \dots \\
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\end{pmatrix}
\]

Where:
\begin{align*}
& T_1 = A_0^p  \ast  B_v0^q  \ast  X_w0^k  \ast  Y_z0 \ast l  \ast  C_{0,v_0}^{kl} \\
& T_2 = A_u^p  \ast  B_v^q  \ast  X_w^k  \ast  Y_z \ast l  \ast  C_{uv}^{kl} \\
& T_3 = A_0^{p+1}  \ast  B_v0^q  \ast  X_w0^k  \ast  Y_z0 \ast l  \ast  C_{0,v0}^{kl} \\
& T_4 = A_u^{p+1}  \ast  B_v^q  \ast  X_w^k  \ast  Y_z \ast l  \ast  C_{uv}^{kl}
\end{align*}

\Eric{need to make sure this survived the conversion to latex without errors}

Subtract the first row times $A_0$ from the second row, and obtain:


\[
\begin{pmatrix}
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\dots & T_1 & \dots & T_2 & \dots \\
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\dots & 0 & \dots & T_4 - A_0 \ast T_2 & \dots \\
 \vdots & \vdots & \vdots & \vdots & \vdots \\
\end{pmatrix}
\]

Where:
\begin{align*}
& T_4 - A_0 \ast T_2 = (A_u-A_0) \ast A_u^p  \ast  B_v^q  \ast  X_w^k  \ast  Y_z \ast l  \ast  C_{uv}^{kl}
\end{align*}


Repeat for all rows in this order: $(m_1-1,q,k,l), (m_1-2,q,k,l),
\dots,(1,q,k,l)$, and for all combinations of $q,k,l$.  Let's examine the
resulting matrix.

Assume that the first $m_2 \ast n_1 \ast n_2$ rows are of the form $(0,q,k,l)$.  Also,
assume that the first $m_2 \ast n_1 \ast n_2$ columns are the form $(0,v,w,z)$
(permute if necessary)

Therefore the matrix looks like this:

\[
\left(
\begin{array}{c|c}
    m_1  &   \dots \\ \hline
    0   &   M'
\end{array}
\right)
\]

In other words:

\begin{itemize}

\item The top-left $m_2 \ast n_1 \ast n_2$ rows and columns are precisely $m_1 =
   M(1,m_2,n_1,n_2)$.  Notice that this matrix does not depend on $A$.

   All entries below it are 0.

\item Therefore, $det(M) = det(m_1)  \ast  det(M')$

   where $M'$ is the bottom right matrix (what remains after removing
   the first $m_2 \ast n_1 \ast n_2$ rows and columns).   This follows from
   a theorem on expanding determinants

\item $M'$ has a factor $(A_u - A_0)$ in every column $(u,v,w,z)$ (this can be
   seen from the big picture above).  Factorize this common factor,
   noting that it occurs $m_2 \ast n_1 \ast n_2$ times (for all combinations of
   $v,w,z$).  Thus:
\[
       det(M') = \prod_u (A_u - A_0)^{m_2 \ast n_1 \ast n_2} det(M'')
\]

   where $M''$ is the matrix resulting from $M'$ after factorizing.

\item The entries of $M''$ are precisely:
\[
    A_u^p  \ast  B_v^q  \ast  X_w^k  \ast  Y_z \ast l  \ast  C_{uv}^{kl}
\]
   where $p=0,\dots,m_1-2$, and $u=1,\dots,m_1-1$ and the other indices have the same
   range as before.  This can be seen from the picture above.

\item Therefore, $M'' = M(m_1-1, m_2, n_1, n_2)$, with the only change that the
   index $u$ is shifted by one.
  
\end{itemize}
  
\end{proof}

Lemma 1 and 2 prove that $det(M) \ne 0$ whenever all the $A$'s, the $B$'s,
the $X$'s, and the $Z$'s are distinct, and all $C_{uv} \ne 0$.  Thus, our
determinant is nonzero, because $C_{uv} = (A_u - 1)(B_v - 1)/(B_v - A_u)$.

Question: What is the complete closed formula for $det(M)$?  We need to
expand the recursion in Lemma 2 and fill in the base cases from Lemma
1. \Eric{To do}

\Eric{Sufficient to simply say this approach generalizes to prove the matrix
is invertible when we have $f_1,f_2,f_3,f_4$ (instead of just $f_1, f_4$ as in
the example)?}

\subsubsection{Algebraic Independence}

\Eric{This section establishes the notion of algebraic independence as a criterion for when
the functions $A$ and $B$ in the expression of probability for our example query $Q$
 can be set independently.}
 
 
\subsubsection{Definitions}
 
Let $Q$ be a query with a single left unary and a single right unary
symbol $U(x), V(y)$.  Let $F$ be its Boolean formula, and denote:
\begin{align*}
& F_{00} = F[0/U, 0/V] \\
& F_{01} = F[0/U, 1/V] \\
& F_{10} = F[1/U, 0/V] \\
& F_{11} = F[1/U, 1/V]
\end{align*}

With some abuse of notation we refer to them as $F_1, F_2, F_3, F_4$.

\begin{fact}Q is splittable iff one of the four functions $F_1, \dots, F_4$ is
unsatisfiable.
\end{fact}
\begin{proof}
If $Q$ is splittable then it has a prime implicate of the form
$((\lnot)U \lor (\lnot)V)$.  Then that corresponding function is 0.  For example,
suppose $Q \Rightarrow (\lnot U \lor V)$.  Then $F_{10} = F[1/U,0/V] = 0$.
\end{proof}


\begin{fact}$Q$ is decomposable iff there exists polynomials $g_0, g_1$ and $h_0,
h_1$ such that the polynomials $f_{00}, f_{01}, f_{10}, f_{11}$ factorize as follows:
\begin{align*}
&   f_{00} = g_0 * h_0 \\
&   f_{01} = g_0 * h_1 \\
&   f_{10} = g_1 * h_0 \\
&   f_{11} = g_1 * h_1 
\end{align*}
\end{fact}
\begin{proof} 
Assume $f_{00}, f_{01}, f_{10}, f_{11}$ factorize as above.  Then we have $f =
(1-u)(1-v) f_{00} + \dots + u v f_{11} = ((1-u) g_0+u g_1) ((1-v) h_0+v h_1)$
proving that $Q$ is decomposable.  The converse is immediate.
\end{proof}

\subsubsection{Outline of General Hardness Proof}

Given a forbidden query $Q$, we prove
hardness by reduction from \#PP2CNF.  Given a PP2CNF formula $\Phi$:
\[
       \Phi = \bigwedge_{(i,j) \in E} (X_i \lor Y_j)
\]

Where $E \subseteq [n] \times [n]$, we set the probabilities as
follows:
\begin{align*}
& P(U(i)) = u \\
& P(V(j)) = v \\
& P(X_1(i,j)) = x_1, P(X_2(i,j) = x_2, \dots if (i,j) \in E \\
& P(X_1(i,j)) = y_1, P(X_2(i,j) = y_2, \dots if (i,j) \not\in E
\end{align*}

Fix an assignment $\theta: \{X_1, \dots, X_n, Y_1, \dots, Y_n\} \rightarrow \{0,1\}$.

Call its parameters the following six numbers:
\begin{align*}
&   k = \text{number of $i$'s s.t. } X_i=1 \\
&   l = \text{number of $j$'s s.t. } Y_j=1 \\
&   q = \text{number of $(i,j) \in E$ s.t. } X_i = 0, Y_j = 0 \\
&   r = \text{number of $(i,j) \in E$ s.t. } X_i = 0, Y_j = 1 \\
&   s = \text{number of $(i,j) \in E$ s.t. } X_i = 1, Y_j = 0 \\
&   p = \text{number of $(i,j) \in E$ s.t. } X_i = 1, Y_j = 1
\end{align*}

Let $N(k,l,q,r,s,p)$ = number of assignments $\theta$ with these parameters.

By repeating the calculations we did for the example query, \Eric{and omitting a constant
factor}, we obtain:
\[
P(Q) = \sum_{k,l,q,r,s,p}  N(k,l,q,r,s,p) A^q  B^r  C^s D^p X^k  Y^l  H^{kl}
\]

Where:
\begin{align*}
&  A = f_{00}(x1,x2, \dots) / f_{00}(y1,y2, \dots) \\
&  B = f_{01}(x1,x2, \dots) / f_{01}(y1,y2, \dots) \\
&  C = f_{10}(x1,x2, \dots) / f_{10}(y1,y2, \dots) \\
&  D = f_{11}(x1,x2, \dots) / f_{11}(y1,y2, \dots) \\
&  H = \text{depends on } A,B,C,D \\
&  X = \text{depends on } A,B,C,D \text{ and } u \\
&  Y = \text{depends on } A,B,C,D \text{ and } v
\end{align*}

As in the example, we use an oracle for $P(Q)$ repeatedly to construct
a system of linear equations and solve for $N(k,l,q,r,s,p)$ in polynomial
time. From here we derive $\#\Phi$.

To do this, we prove that the matrix $M$ of the resulting system has
$det(M) \ne 0$.

The same reduction of the matrix to a product of Vandermonde matrices
applies as with our example query, as long as we can produce distinct 
values for $A, B, C,$ and $D$. This establishes the following:

\begin{fact} Consider four sequences of m+1 distinct
numbers:
\begin{align*}
&   A_u, u=0,\dots,m \\
&   B_v, v=0,\dots,m \\ 
&   C_w, w=0,\dots,m \\
&   D_z, z=0,\dots,m
\end{align*}

Suppose that for every combination of $u,v,w,z$ we can find
probabilities $x_1, x_2, \dots, y_1, y_2, \dots$ s.t.  $A_u =
f_{00}(x_1,x_2,\dots)/f_{00}(y_1,y_2,\dots)$, 
$B_v = f_{01}(x_1,x_2,\dots)/f_{01}(y_1,y_2,\dots)$, etc.
Then $det(M) \ne 0$.
\end{fact}


Thus, to prove that $P(Q)$ is \#P-hard it suffices to prove that the four
functions $A, B, C, D$ are invertible: that is, given their output
values $A_u, \dots, D_z$, we must find inputs $x_1,x_2, \dots,y_1,y_2,\dots$ s.t. 
when the functions are applied to those inputs they result in the desired
values.

Clearly, $A,B,C,D$ are not invertible in two trivial cases: when some of
the functions $f_{00},f_{01},f_{10},f_{11}$ are constants, or when two or more are
equivalent.  The case analysis (see section \ref{subset:case analysis}) establishes that
these cases can either be handled by grouping identical functions and ignoring
constantly true functions, as with our example query. As another example, 
suppose $f_{01} = 1$, then we remove $r$ from the statistics, i.e. $N$
becomes $N(k,l,q,s,p)$.  Knowing all values of $N(k,l,q,s,p)$ still
allows us to compute $\#\Phi$. Alternately, the case analysis shows that the queries
where we cannot invert $A,B,C,D$ are exactly the queries amenable to our second
hardness proof technique, the zigzag construction.

Thus, we will assume that the four functions $F_{00}, F_{01}, F_{10}, F_{11}$ are
non-constant and inequivalent.  Then, the hardness proof follows
from the following theorem:


\ifx true false


\begin{theorem}
Let $Q$ be a forbidden query with two unary atoms $U, V$.
Suppose the four functions $F_{00}, \dots, F_{11}$ are distinct and non-constant.
Note that this implies that there are at least two variables $x_1, x_2$.  Then the
Jacobian of the four functions $A, B, C, D$ has rank 4.

PROOF.  I will denote the four functions f1(x), f2(x), f3(x), f4(x),
where x= (x1, x2, ...) is the set of variables.  Further denote
g1(y)=f1[y/x], .., g4(y) = f4[y/x], where y=(y1,y2,..) are fresh
variables.  Recall that:

   A = f1(x) / g1(y)
   B = f2(x) / g2(y)
   C = f3(x) / g3(y)
   D = f4(x) / g4(y)

Their Jacobian has the same rank as the Jacobian of their log, which
is:

  log(A) = log(f1)  -  log(g1)
  log(B) = log(f2)  -  log(g2)
  log(C) = log(f3)  -  log(g3)
  log(D) = log(f4)  -  log(g4)

The Jacobian matrix looks like this:

  1/f1*d(f1)/d(x1)  1/f1*d(f1)/d(x2) ... -1/g1*d(g1)/d(y1) ...
  ..
  1/f4*d(f1)/d(x1)  1/f4*d(f1)/d(x2) ... -1/g4*d(g1)/d(y1) ...

Each column corresponding to a y-variable has a minus sign.  Revert
that sign (it doesn't change the rank of the matrix), and we obtain
the Jacobian of these four functions:

    log(f1) + log(g1)
    ...
    log(f4) + log(g4)

The theorem follows from the following proposition:

PROPOSITION.  Let f1(x), .., f4(x) be the four functions of a
forbidden query, and g1(y), .., g4(y) obtained by substituting y for
x.  Assume f1,..,f4 are not constant, and no two are equivalent.  Then
the Jacobian of f1*g1, f2*g2, f3*g3, f4*g4 has rank 4.

 NOTE. We have a somewhat elegant way to prove the proposition by
 reducing it to a number of special cases, maybe about 20 or so; we
 have not checked all these special cases yet, but they seem
 straightforward.  Both Eric and I believe that there must be a
 simpler argument, in particular one that reduces to fewer special
 cases.  (My current conjecture is this: if f1, ..., f4 are four
 functions and g1, ..., g4 their clones, and if f1*g1, .., f4*g4 has
 rank less than 4, then there exists five constants c1,..,c4, c such
 that the following identity holds: c1*log(f1) + .. + c4*log(f4) = c.
 Thus, the only special cases would be f1*f4=f2*f3 (which I can prove
 implies Q is decomposable), or f1*f2=f3 (which can be shown is
 hard).)   But for now all we have is the proof below.  The good news
 is that the math that we used is really cool.


The proof of the proposition uses the following background on
multivariate polynomials:

 BACKGROUND:

   DEFINITION.  Let f1, ..., fn be multivariate polynomials. An
   "anihilating polynomial" is a polynomial A(z1,..,zn) such that the
   following identity holds:  A(f1,...,fn) = 0.

   Clearly, if f1,..,fn have an anihilating polynomial, then the Jacobian determinant
   Det(J(f1,..,fn))=0 everywhere.  Otherwise they are called
   "algebraically independent".

   PROPOSITION. If f1, ..., fn are over n-1 variables, then they have
   an anihilating polynomial.  (Note: this is easy to prove
   directly.)

   PROPOSITION. If f1, ..., fn have an anihilating polynomial, and
   any n-1 are algebraically independent, then there exists a unique
   irreducible anihilating polynomial A for f1, ..,fn.

   (And, does it follow that any other anihilating polynomial divides
   A?  Unclear...)

   PROPOSITION. If the Jacobian J(f1,...,fn) has rank < n, then f1,
   ..., fn have an anihilating polynomial.

   (I find this incredibly cool.  The implicit function theorem tells
   us that if J(f1,...,fn) = 0 on an open set, then there exists an
   "implicit function" F s.t. F(f1,..,fn) = 0 on an open set.  For
   polynomials, the implicit function can be chosen to be another
   polynomial!  We found a paper with a very simple, and non-obvious
   proof.)

   It is very instructive to play with anihilating polynomials for
   the four Boolean functions resulting from a query Q.

   EXAMPLE 1 If Q decomposes: f1=g0*h0, f2=g0*h1, f3=g1*h0, f4=g1*h1,
   and the anihilating polynomial is A = f1*f4 - f2*f3 = 0.

   EXAMPLE 2. Suppose f1 = x1 + x2 - x1*x2, f2 = x1*x2, f3=x1.  Then
   A = (f1 + f2 - f3)*f3 - f2 = 0

   We also need the following: (1) The ideal generated by f1, .., fn,
   denoted <f1,..,fn, is the set of polynomials of the form f1*h1 +
   ... fn*hn, for arbitrary h1, ..., hn.  (2) The variety of an ideal
   I is V(I) = {a | for all f \in I, f[a/x] = 0}. In particular,
   V(f1,..,fn) is the variety of <f1,..,fnand consists of all
   common roots of f1,..fn. (3) Hilbert's Nullstellensatz: if V(I)
   \subseteq V(f) then there exists m s.t. f^m \in I.  We only need a
   very simple consequence: if p is irreducible and V(p) \subseteq
   V(f), then f \in <p, in other words f is divisible by p.


I will now prove the proposition.  I will change the notations of g1,
..,g4 to k1,..k4:

Let f1(x), .., f4(x) be four polynomials in variables x, and k1(y),
..., k4(y) be four polynomials in variables y (disjoint from x).

The key step is this:

LEMMA.  Suppose there exists two factors p \in Factors(f3), q \in
Factors(f4) such that the following hold:

   (a)   V(q) \not\subseteq V(f3)
   (b)   V(p,q) \not\subseteq V(f1) \cup V(f2)

If k1, k2 are algebraically independent, then f1*k1, ..., f4*k4 are
algebraically independent.

PROOF Suppose the contrary: there exists an anihilating polynomial:

   A(f1*k1, ..., f4*k4) = 0

From (b) we derive that there exists some value a in V(p,q) such that:

    f1[a/x] != 0, f2[a/x] != 0, f3[a/x] = f4[a/x] = 0

From (a) and (be) we derive that V(q) is not included in V(f1) \cup
V(f2) \cup V(f3): otherwise V(q) \subseteq V(f1*f2*f3) then by
Hilbert's Nullstellensatz: (f1*f2*f3)^m \in <q, hence q is a factor
of (f1*f2*f3)^m, hence it is a factor of either f1, f2, or f3,
violating either (b) or (a)  Thus, there exists a value b \in V(q)
such that:

    f1[b/x] != 0, f2[b/x] != 0, f3[b/x] != 0, f4[b/x] = 0

We claim that it is possible to choose a and b such that they are
consistent, in other words we claim that p[b/x] has some free
variables (not set by b) such that we can obtain a by setting those
variables to some constants.

This is actually best done using the quotient construction.  If R[x]
denotes the ring of multivariate polynomials over x, then R[x]/q(x) is
the quotient ring.

For any polynomial f(x) \in R[x], its equivalence class is denoted
[f(x)] \in R[x]/q(x).  "Setting q=0" means, technically, replacing
every polynomial f with [f].  Note that [q(x)] = 0, which implies
[f4]=0, and we have [f1], [f2], [f3] != 0, because V(q) is not a
subset of V(f1*f2*f3).

For a polynomial F(x,y) \in R[x,y], its equivalence class [F(x,y)] is
obtained by writing F as a sum of monomials:

   F = sum_e C_e(x) * y^e

then [F(x,y)] = sum_e [C_e(x)] * y^e.  Therefore, [f1*k1]=[f1]*k1 etc.

Denoting B(z1,z2,z3) = A(z1,z2,z3,0), we cannot have B==0 because then
A would be reducible.  Thus:

0 =  [A(f1*k1, .., f4*k4)] = A([f1]*k1, [f2]*k2, [f3]*k3, 0)
                          = B([f1]*k1, [f2]*k2, [f3]*k3)
                          = B1([f1]*k1, [f2]*k2, [f3]*k3)

Since B([f1]*k1,...) is identical 0, there exists an irreducible
polynomial B1 s.t. B1([f1]*k, ...) is identical 0.

Next, we "set [p]=0".  Formally, we obtain this by constructing the
new quotient ring (R[x]/<q)/<p, and mapping every polynomial [f] to
[[f]].  We have [[p]]=0, hence [[f3]]=0.  We claim that [[f1]], [[f2]]
!= 0.  Indeed, suppose [[f1]]=0, then [f1] \in <[p], which is
equivalent to f1 \in <p,q, but this contradicts (b).  Therefore:

0 = B1([[f1]]*k1, [[f2]]*k2, [[f3]]*k3) = B1([[f1]]*k1, [[f2]]*k2, 0)

Since [[f1]], [[f2]] are non-zero, we can substitute all their
variables with constants s.t. [[f1]] = c1 != 0, [[f2]] = c2 != 0:

0 = B1(c1*k1, c2*k2, 0)

Contradiction.

END OF THE PROOF OF THE LEMMA.

Continuing the proof of the proposition, we have proven the claim in
the proposition for all queries EXCEPT for queries that do not satisfy
the conditions in the lemma.  In other words they satisfy:

 forall q \in Factors(f4) - Factors(f3),
    forall p \in Factors(f3),
       V(p,q) \subseteq V(f1*f2)

and all conditions obtained by permuting f1,f2,f3,f4.

Let:

  F3' = Factors(f3) - Factors(f4)
  F4' = Factors(f4) - Factors(f3)
  F34 = Factors(f3) \cap Factors(f4)

The condition is further equivalent to:

  forall p in F3, q in F4', V(p,q) \subseteq V(f1*f2)

and permuting F3, F4:

  forall p in F3', q in F4, V(p,q) \subseteq V(f1*f2)

The two conditions above are equivalent to these three:

   forall p in F3', q in F4', V(p,q) \subseteq V(f1*f2)
   forall p in F3', q in F34, V(p,q) \subseteq V(f1*f2)
   forall p in F34, q in F4', V(p,q) \subseteq V(f1*f2)

In the last two cases p,q have disjoint sets of variables.  I will
prove the following:

CLAIM. If p, q, are irreducible polynomials over disjoint sets of
variables, then V(p,q) \subseteq V(f*g) iff V(p,q) \subseteq V(f) or
V(p,q) \subseteq V(g).

Intuitively, the claim generalizes the fact that: V(p) \subseteq
V(f*g) implies V(p) \subseteq V(f) or V(p) \subseteq V(g) (because
V(p) \subseteq V(f*g) implies that p divides f*g, hence it divides
either f or g, because it is irreducible).  I will prove the claim
below.  For now, I will show how to use it:

By applying this argument repeatedly we obtain V(p,q) \subseteq V(r),
where r is some factor of f1 or f2.  Therefore, the conditions become:

(I will abuse notation and write F1 instead of Factors(F1)).

forall p in F3', q in F34, either (p \in F1 \cup F2) or (q \in F1 \cup F2)
forall p in F34, q in F4', either (p \in F1 \cup F2) or (q \in F1 \cup F2)

The two conditions are equivalent to:

 (F3' \subseteq F1 \cup F2) or (F34 \subseteq F1 \cup F2)
 (F34 \subseteq F1 \cup F2) or (F4' \subseteq F1 \cup F2)

Indeed, suppose otherwise, i.e. there exists p \in F3' and q \in F34
s.t. neither p nor q are in F1 \cup F2: then the first condition above
fails too.

Applying distributivity, they are equivalent to:

     [(F3' \subseteq F1 \cup F2) and (F4' \subseteq F1 \cup F2)]
 or  [F34 \subseteq F1 \cup F2]

In other words, the proposition fails only on queries that satisfy the
following three conditions, and all conditions obtained by permuting
F1, ..., F4:

      (C1) F3  \subseteq F1 \cup F2
           or
      (C2) F4  \subseteq F1 \cup F2
           or
      (C3) Delta(F3,F4) \subseteq F1 \cup F2


We can now describe all cases of queries where the assumptions in the
LEMMA fail.  These are the queries where we need to prove hardness
directly, either by simply showing that f1*k1,..., f4*k4 are
algebraically independent, or by some other means.

CASE 1. There exists an irreducible factor w that occurs in only one
       of the four functions F1, .., F4.  Assume wlog that w \in F4.
       Then (C1) must hold, under all permutations of F1, F2, F3.
       This implies that every factor that occurs in F1, F2, F3
       occurs in at least two of them.  Therefore, these functions
       look like this:


       F1 = p * q  * s
       F2 = p * r  * s
       F3 = q * r  * s
       F4 = w * ...

       That is, p contains all factors that occur in both F1 and F2,
       etc, and w occurs only in F4.  For example:

       F1 = x1 * x2 * (1-x3)
       F2 = x1 * (1-x3)
       F3 = x2 * (1-x3)
       F4 = x3

       (In this example we prove the proposition directly, by showing
       that the Jacobian of F1*K1, ..., F4*K4 on the variables x1,
       x3, y2, y3 is non-zero.)

CASE 2. Every factor occurs in two or more functions.  Then the
       functions look like this:

       F1 = p * q * r * [rest]
       F2 = p * s * t * [rest]
       F3 = q * s * r * [rest]
       F4 = r * t * r * [rest]

       where p consists of all factors that occur in both F1 and F2,
       etc, and [rest] represents factors that occur in three or more
       functions.

That's as far as we got in the "case analysis".

Finally, I prove the claim above:

LEMMA.  Let p(x), q(y) be irreducible polynomials, over disjoint sets
of variables x and y respectively.  Suppose V(p,q) \subseteq V(f1*f2)
where f1(x,y), f2(x,y) are arbitrary polynomials.  Then at least one
of the following holds:
  V(p,q) \subseteq V(f1), or
  V(p,q) \subseteq V(f2).

PROOF.  Notice that V(p,q) = {(a,b)| p(a) = 0 and q(b) = 0}.  In other
words, V(p,q) is the cartesian product V(p) x V(q), and the assumption
of the lemma is:

  forall a \in V(p), forall b \in V(q) ==(a,b) \in V(f1*f2).

We claim:

(*)  forall a in V(p):
       either q divides f1[a/x] or
       or     q divides f2[a/x]

Indeed, if a \in V(p), then:

   {a} \times V(q) \subseteq V((f1*f2)[a/x])

hence q divides f1[a/x]*f2[a/x], hence it either divides f1[a/x] or
divides f2[a/x] (because it is irreducible).

We claim that the following stronger property holds:

(**)   either: forall a in V(p), q divides f1[a/x]
      or:     forall a in V(p), q divides f2[a/x]

This claim proves the lemma, because in the first case V(p,q)
\subseteq V(f1), and in the second case V(p,q) \subseteq V(f2).

We prove (**) by using the "remainder of dividing f1(x,y) by q(y)",
which we denote g1.  In other words:

 (1)      g1(x,y) = sum_e c_e(x) y^e

where every exponent sequence e for y is "smaller" than the
multidegree of g.

    Formally, following the notations in Giesbrecht's lecture on
    Multivariate Polynomials and Grobner basis: fix an admissible
    monomial order <, then g1 is the normal form of f1 w.r.t. p, that
    is f1 --^{*}_{q} g1 and there is no h s.t. g1 --_{q} h.

Similarly, let g2(x,y) be the remainder of dividing f2 by q:

  (2)      g2(x,y) = sum_{e'} d_{e'}(x) y^{e'}

From (*) we have:

(+)  forall a in V(p):
       either forall e,  c_e[a/x] = 0
       or     forall e', d_{e'}[a/x] = 0

This implies:

   forall a in V(p), forall e, e' c_e[a/x]*d_{e'}[a/x] = 0

equivalently:

   forall e, e', forall a in V(p),  c_e[a/x]*d_{e'}[a/x] = 0

still equivalently:

   forall e, e': p(x) divides c_e(x) * d_{e'}(x)

Since p(x) is irreducible, it implies that either p(x) divides c_e(x)
or it divides d_{e'}(x).  We claim that the following holds:

(++)   either: forall e, p(x) divides c_e(x)
      or:     forall e', p(x) divides d_{e'}(x)

Suppose not: then there exists e such that p(x) does not divide c_e(x)
and there exists e' such that p(x) does not divide d_{e'}(x),
contradiction, because we know that p(x) must divide one of c_e(x) or
d_{e'}(x).  Property (++) immediately implies (**).

QED.

The requirement that p, q have disjoint sets of variables is
necessary.  Otherwise, consider:

  p = xyz + xy + x + y + 2
  q = xyz + 1

  f1 = x+1
  f2 = y+1

Then p-q = xy + x + y + 1 = (x+1)*(y+1) = f1*f2

This implies V(p,q) \subseteq V(f1*f2), but V(p,q) is not a subset of
V(f1), because any triple of the form (a,b,c) with a*b=1, c=-1 is in
V(p,q) but it is not in V(f1) (for example (a,b,c) = (3, 1/3, -1) \in
V(p,q) but not in V(f1)).  Similarly, V(p,q) is not in V(f2)


\fi


 

\subsubsection{Zigzag Construction}

\Eric{The zigzag construction is a method from \citep{dalvi2012dichotomy} that
replaces $Q$ with a structure $Q' = Q_1 \land Q_2 \land Q_3 \land Q_4 \land Q_5$
such that computing $P(Q)$ in polynomial time implies the ability to calculate
$P(Q')$ in polynomial time, and $\#\Phi \le_p P(Q')$. The construction requires
that we only consider specific tuples between $Q_i$ and $Q_{i+1}$, which is only
possible in certain cases. The case analysis of the next section shows that all
queries of type 1 with one left and one right unary symbol where our algorithm gets
stuck can either be shown to be hard through the algebraic independence or the zigzag
method.}

\subsubsection{Case Analysis}
\label{subset:case analysis}

\Eric{Here we have the lemma about algebraic varieties and algebraic independence
and the case analysis showing that any queries where the lemma fails admit the
zigzag construction.}











